Going Full-TILT Boogie on Document Understanding with Text-Image-Layout Transformer

We address the challenging problem of Natural Language Comprehension beyond plain-text documents by introducing the TILT neural network architecture which simultaneously learns layout information, visual features, and textual semantics. Contrary to previous approaches, we rely on a decoder capable of unifying a variety of problems involving natural language. The layout is represented as an attention bias and complemented with contextualized visual information, while the core of our model is a pretrained encoder-decoder Transformer. Our novel approach achieves state-of-the-art results in extracting information from documents and answering questions which demand layout understanding (DocVQA, CORD, SROIE). At the same time, we simplify the process by employing an end-to-end model.

==> abstract.tex <==
Sample abstract.


==> autozoil-extras.tex <==

\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\noqa}[1]{}
\newcommand{\noqall}[1]{}



==> config.tex <==
% In this file some settings are passed from cookiecutter to LaTeX.
% Do not edit this file, but rather change .cookiecutter.yml and
% re-apply the template.

% whether an appendix was created
\newif\ifwithappendix
\withappendixfalse


% whether the appendix will actually be shown;
% note: in some template, the appendix cannot be rendered,
% you can use this conditional to change the content of your paper
% (for instance, to remove parts like "see Appendix")
\newif\ifappendixshown
\appendixshowntrue



==> extras.tex <==


\input{other-extras}
\input{autozoil-extras}

%%% Local Variables:
%%% mode: latex

%%% TeX-master: "l5"
%%% End:


==> keywords.tex <==
some keyword, another keyword


==> metadata.tex <==
\title{L5 paper}

\author{\bf First Author \\
  Affiliation / Address line 1 \\
  Affiliation / Address line 2 \\
  Affiliation / Address line 3 \\
  \texttt{email@domain} \\
  \and \bf Second Author \\
  Affiliation / Address line 1 \\
  Affiliation / Address line 2 \\
  Affiliation / Address line 3 \\
  \texttt{email@domain} \\}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "l5"
%%% End:


==> other-extras.tex <==

% various custom definitions

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[textsize=tiny]{todonotes}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{latexsym}

% so that footnotes in tables would work
% https://tex.stackexchange.com/questions/109467/footnote-in-tabular-environment

\usepackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}
\makesavenoteenv{table*}

% for better typesetting of URLs

\usepackage{xurl}

% input without unwanted end-of-line characters

\newcommand\minput[1]{%
  \input{#1}%
  \ifhmode\ifnum\lastnodetype=11 \unskip\fi\fi}

% Gonito stuff
\usepackage{hyperref}
\usepackage{xstring}
% Format a reference to a Gonito submission
\newcommand{\gonitoref}[1]{\{\href{https://gonito.net/q/#1}{\StrMid{#1}{1}{6}}\}}
% A bare score from Gonito
\newcommand{\gonitobarescore}[1]{\minput{scores/#1.txt}}
% A score from Gonito along with a reference
\newcommand{\gonitoscore}[1]{\gonitobarescore{#1} \gonitoref{#1}}
% A reference and a score as two cells in a table
\newcommand{\gonitoentry}[1]{\gonitoref{#1} & \minput{scores/#1.txt}}



==> preamble.tex <==

% extra packages and definitions

\usepackage{amsmath}

